Axion search with BabyIAXO in view of IAXO

Axions are a natural consequence of the Peccei-Quinn mechanism, the most compelling solution to the strong-CP problem. Similar axion-like particles (ALPs) also appear in a number of possible extensions of the Standard Model, notably in string theories. Both axions and ALPs are very well motivated candidates for Dark Matter, and in addition, they would be copiously produced at the sun's core. A relevant effort during the last decade has been the CAST experiment at CERN, the most sensitive axion helioscope to-date. The International Axion Observatory (IAXO) is a large-scale 4th generation helioscope. As its primary physics goal, IAXO will look for solar axions or ALPs with a signal to background ratio of about 5 orders of magnitude higher than CAST. Recently the IAXO collaboration has proposed and intermediate experimental stage, BabyIAXO, conceived to test all IAXO subsystems (magnet, optics, detectors and sun-tracking systems) at a relevant scale for the final system and thus serve as pathfinder for IAXO but at the same time as a fully-fledged helioscope with record and relevant physics reach in itself with potential for discovery. BabyIAXO was endorsed by the Physics Review committee of DESY last May 2019. Here we will review the status and prospects of BabyIAXO and its potential to probe the most physics motivated regions of the axion & ALPs parameter space.

==> authors.tex <==
%% In this file we only define variables (affiliations, index superscripts, and the list of authors and the list of institutions) %%

%% First of all, define the upperscripts associated to each affiliation (easily changed depending on the article, proceeding,...
%% Add one line per institution with this format:
%% \newcommnad{\INSTITUTIONACRONYM}{$^{SUPERSCRIPT}$}


\newcommand{\UHEI}{1}
\newcommand{\UNIZAR}{2}
\newcommand{\CERN}{3}
\newcommand{\CEAIrfu}{4}
\newcommand{\INAF}{5}
\newcommand{\IJCLAB}{6}
\newcommand{\MIPT}{7}
\newcommand{\INR}{8}
\newcommand{\DTU}{9}
\newcommand{\ICCUB}{10}
\newcommand{\UBFQA}{11}
\newcommand{\PNPI}{12}
\newcommand{\UBonn}{13}
\newcommand{\USiegen}{14}
\newcommand{\BARRY}{15}
\newcommand{\JENA}{16}
\newcommand{\Columbia}{17}
\newcommand{\CEFCA}{18}
\newcommand{\SOLEIL}{19}
\newcommand{\RBI}{20}
\newcommand{\DESY}{21}
\newcommand{\CEAList}{22}
\newcommand{\ICREA}{23}
\newcommand{\MIT}{24}
\newcommand{\SLAC}{25}
\newcommand{\Mainz}{26}
\newcommand{\UCT}{27}

%% Now define the full address text of each affiliation
%% add a line per institution with the following format:
%% \newcommand{\INSTITUTIONACRONYMname}{FULL_NAME_AND_ADDRESS_OF_INSTITUTION}

\newcommand{\UNIZARname}{Center for Astroparticles and High Energy Physics (CAPA), Universidad de Zaragoza, 50009 Zaragoza, Spain}
\newcommand{\BARRYname}{Physical Sciences, Barry University, 11300 NE 2nd Ave., Miami Shores, FL 33161, USA}
\newcommand{\MITname}{Massachusetts Institute of Technology, 77 Massachusetts Ave., Cambridge, MA 02139, USA}
\newcommand{\CEFCAname}{Centro de Estudios de F\'{\i}sica del Cosmos de Arag\'on, Plaza San Juan, Teruel, Spain}
\newcommand{\ICCUBname}{Institut de Ci\`encies del Cosmos, Universitat de Barcelona, Barcelona, Spain}
\newcommand{\UBFQAname}{Departament de F\'isica Qu\`antica i Astrof\'isica, Universitat de Barcelona, Barcelona, Spain}
\newcommand{\ICREAname}{ICREA, Barcelona, Spain}
\newcommand{\Mainzname}{Johannes Gutenberg University, Mainz, Germany}
\newcommand{\PNPIname}{Petersburg Nuclear Physics Institute - NRC Kurchatov Institute, Gatchina, 188300, Russia}
\newcommand{\RBIname}{Rudjer Bo\v{s}kovi\'{c} Institute, Bijeni\v{c}ka cesta 54, 10000 Zagreb, Croatia}
\newcommand{\UBonnname}{Physikalisches Institut der Universit\"at Bonn, Nussallee 12, 53115 Bonn, Germany}
\newcommand{\UCTname}{High Energy Physics, Cosmology \& Astrophysics Theory (HEPCAT) group, University of Cape Town, Private Bag, 7700 Rondebosch, South Africa}
\newcommand{\DESYname}{Deutsches Elektronen-Synchrotron DESY, Hamburg, Germany}
\newcommand{\CERNname}{CERN - European Organization for Nuclear Research, Geneva, Switzerland}
\newcommand{\UHEIname}{Heidelberg University, Kirchhoff Institute for Physics}
\newcommand{\LLNLname}{Lawrence Livermore National Laboratory, Livermore, CA, U.S.A.}
\newcommand{\Columbianame}{Columbia Astrophysics Laboratory, New York, U.S.A.}
\newcommand{\DTUname}{Technical University of Denmark, DTU Space Kgs. Lyngby, Denmark}
\newcommand{\SLACname}{SLAC National Accelerator Laboratory, Menlo Park, CA, U.S.A.}
\newcommand{\JENAname}{Institute  for  Optics  and  Quantum  Electronics,  Friedrich  Schiller  University  Jena,  Jena,  Germany}
\newcommand{\INAFname}{INAF, Italian National Institute for Astrophysics, Osservatorio Astronomico di Brera, Milano/Merate, Italy}
\newcommand{\INRname}{Institute  for Nuclear Research of the Russian Academy of Sciences, 60th October Anniversary Prospect 7A, 117312, Moscow, Russia}
\newcommand{\USiegenname}{Center for Particle Physics Siegen, Siegen University, Siegen, Germany}
\newcommand{\CEAIrfuname}{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\newcommand{\CEAListname}{CEA, LIST, Laboratoire National Henri Becquerel (LNE-LNHB), F-91191 Gif-sur-Yvette, France}
\newcommand{\MIPTname}{Moscow Institute of Physics and Technology, Moscow, Russia}
\newcommand{\IJCLABname}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\SOLEILname}{Synchrotron SOLEIL, 91192 Gif-sur-Yvette, France }


\author[\UHEI]{A.~Abeln}
\author[\UNIZAR]{K.~Altenm\"uller}
\author[\CERN]{S.~Arguedas Cuendis}
\author[\CEAIrfu]{E.~Armengaud}
\author[\CEAIrfu]{D.~Atti\'e}
\author[\CEAIrfu]{S.~Aune}
\author[\INAF]{S.~Basso}
\author[\IJCLAB]{L.~Berg\'e}
\author[\CEAIrfu]{B.~Biasuzzi}
\author[\CERN]{P.~T.~C.~Borges~De~Sousa}
\author[\CEAIrfu]{P.~Brun}
\author[\CERN]{N.~ Bykovskiy}
\author[\CEAIrfu]{D.~Calvet}
\author[\UNIZAR]{J.~M.~Carmona}
\author[\UNIZAR]{J.~F.~Castel}
\author[\UNIZAR]{S.~Cebri\'an}
\author[\MIPT,\INR]{V.~Chernov}
\author[\DTU]{F.~E.~Christensen}
\author[\INAF]{M.M.~Civitani}
\author[\ICCUB,\UBFQA]{C.~Cogollos}
\author[\UNIZAR]{T.~Dafni}
\author[\PNPI]{A.~Derbin}
\author[\UBonn]{K.~Desch}
\author[\UNIZAR]{D.~D\'iez}
\author[\DESY]{M.~Dinter}
\author[\CERN]{B.~D\"obrich}
\author[\PNPI]{I.~Drachnev}
\author[\CERN]{A.~Dudarev}
\author[\IJCLAB]{L.~Dumoulin}
\author[\DTU]{D.~D.~M.~Ferreira}
\author[\CEAIrfu]{E.~Ferrer-Ribas}
\author[\USiegen]{I.~Fleck}
\author*[\UNIZAR]{J. Galan}
\author[D.~Gasc\'on\ICCUB$^,$\UBFQA,
\author[L.~Gastaldo\UHEI, 
\author[M.~Giannotti\BARRY,
\author[[\CEAIrfu]{Y.~Giomataris\CEAIrfu,
\author[A.~Giuliani\IJCLAB,
\author[S.~Gninenko\INR,
\author[J.~Golm\CERN$^,$\JENA,
\author[N.~Golubev\INR,
\author[L.~Hagge\DESY,
\author[J.~Hahn\USiegen,
\author[C.~J.~Hailey\Columbia,
\author[D.~Hengstler\UHEI,
\author[P.~L.~Henriksen\DTU, 
\author[R.~Iglesias-Marzoa\CEFCA,
\autho



\note{For the IAXO collaboration.}
